"Previously on ..." From Recaps to Story Summarization

We introduce multimodal story summarization by leveraging TV episode recaps - short video sequences interweaving key story moments from previous episodes to bring viewers up to speed. We propose PlotSnap, a dataset featuring two crime thriller TV shows with rich recaps and long episodes of 40 minutes. Story summarization labels are unlocked by matching recap shots to corresponding sub-stories in the episode. We propose a hierarchical model TaleSumm that processes entire episodes by creating compact shot and dialog representations, and predicts importance scores for each video shot and dialog utterance by enabling interactions between local story groups. Unlike traditional summarization, our method extracts multiple plot points from long videos. We present a thorough evaluation on story summarization, including promising cross-series generalization. TaleSumm also shows good results on classic video summarization benchmarks.

==> sections/F_UserStudy.tex <==
\subsection{Human Evaluation and User Study}
\label{sup_sec:user_study}

In this section, we discuss a couple ways to evaluate story summaries.
The first is based on summarized plot synopses from a \tf{} fan site\footnote{\url{https://24.fandom.com/wiki/Wiki_24}} that includes the key events in the story (as a text description).
The second involves showing some users summaries generated through various methods and obtaining ranking and qualitative feedback.

\subsection{Evaluation based on Plot Synopses}

\input{sections/tables/supplementary/compare}

Plot synopses are a short textual description of the key story events of an episode.
We ask annotators to use the plot synopses and tag the start-end duration for story sequences corresponding to the description.
We refer to these labels as \emph{Fandom} and use them for quantitative and qualitative evaluation.

\paragraph{Quantitative evaluation.}
We compare performance of the recap matching process without and with smooth labels, denoted as MR and MRS respectively against the Fandom labels in Table~\ref{tab:compare}.
From rows 1 and 2, we see that the smoothing process improves story summarization performance on the Fandom labels by around 11\% for video shots and 17\% for dialog utterances, resulting in a respectable AP score above 50.

Note, that we also include the evaluation on validation and test episodes, as included in Table 6 of the main paper.
We observe that our model \modelname{} (row 6) is able to achieve the highest performance on Fandom labels as compared to video only baselines (rows 3-5).

\paragraph{Qualitative evaluation.}
We present importance scores for three episodes: S07E22, S06E22, and S06E20 in  Fig.~\ref{fig:three_eps}.
Note, S07E22 was also included as an example qualitative result in Fig.~3 of the main paper.
We observe that the model predictions are quite good and not only match the smoothed matched recap labels (on which the model is trained), but also the human annotations in the form of Fandom labels.


\begin{figure*}
\centering
\includegraphics[width=\textwidth]{figures/supplementary/vid_24-S07E22.pdf}
\includegraphics[width=\textwidth]{figures/supplementary/dia_24-S07E22.pdf}
\includegraphics[width=\textwidth]{figures/supplementary/vid_24-S06E22.pdf}
\includegraphics[width=\textwidth]{figures/supplementary/dia_24-S06E22.pdf}
\includegraphics[width=\textwidth]{figures/supplementary/vid_24-S06E20.pdf}
\includegraphics[width=\textwidth]{figures/supplementary/dia_24-S06E20.pdf}
\caption{Importance scores for video shots and dialog utterances across multiple evaluation episodes of the series \tf.
\emph{y}-axis denotes importance scores while \emph{x}-axis denotes time (in seconds).
We show:
(i)~model predictions in green;
(ii)~story summary labels from a human annotator translating the Fandom textual synopses to intervals in the video in orange; and
(iii)~soft labels derived from matching shots of the recap to the episode in blue.
\emph{Note}: We create this plot by identifying the mid-timestamp for each video shot and dialog utterance and performing cubic-spline based smoothing.}
\label{fig:three_eps}
\end{figure*}


\subsection{Details of the User Study}
We ask three users to participate and watch summaries for three episodes (same episodes as shown in Fig.~\ref{fig:three_eps}).
In the following, we describe the setup of the study and summarize the findings.

\paragraph{User study setup.}
We briefed the users about the general storyline and character information of the TV series \tf{} before starting this study.
Each individual was asked to watch three episodes in their entirety,
give quality ratings (from 1 to 5) for three video summaries associated with each episode and answer some questions related to that.

\input{sections/tables/supplementary/response_table}


The three videos were as follows:
(i)~$\text{S}_\text{M}$: Summary story generated by our model;
(ii)~$\text{S}_\text{I}$: summary generated by stitching randomly selected video intervals; and
(iii)~$\text{S}_\text{R}$: summary generated by randomly selected shots totaling to a specific time duration.

We shuffle and de-identify the order of the short video summaries. 
After rating the videos, we request the participants to answer a few questions:
\begin{enumerate}[nosep]
\item [(a)] Which summary do you think is generated by \modelname{} and why?
\item [(b)] Which summary is produced by a human and why?
\item [(c)] Which summary is obtained by randomly stitching shots and why?
\end{enumerate}

Note, (b) is a trick question for our study, as none of the shown summaries are produced by humans.


\paragraph{User study findings}
are presented in the Table~\ref{tab:response_table}.
In the top half, we see that 5 of 9 responses rank the model-generated video summary as the best.
Interestingly, the choosing of random intervals as done in $\text{S}_\text{I}$ is a hard baseline since crisply edited videos often contain important storylines all through the episode, and including them in the summary results in acceptable summaries.
The average rank (lower is better) for the three videos can be summarized as:
1.56 for model predictions $\text{S}_\text{M}$;
1.78 for the summary with contiguous story intervals $\text{S}_\text{I}$; and
2.44 for the random selection of shots $\text{S}_\text{R}$.


The bottom half of the table indicates which video is selected for each question.
Q(a) regarding which video is model generated is answered correctly 4/8 times as the users often pick the model generated summary.
Q(c) asks about which video is randomly stitched. Here we see that users are easily able to pick out the randomly stitched video 6/7 times.
Finally, Q(b) is the interesting question as it asks about which summary is human generated, while no summaries are actually human generated.
Here, users pick the model generated summary 5/8 times indicating a strong preference for our model's predictions.


\paragraph{Supplementary videos.}
In the supplementary file, we attach example summary videos from our model and ones generated by humans based on the Fandom plot synopses for two episodes.
Note the video quality is quite poor as we were forced to compress them to fit in the supplementary material size limit.

